Community Detection Using Slow Mixing Markov Models

The task of \emph{community detection} in a graph formalizes the intuitive task of grouping together subsets of vertices such that vertices within clusters are connected tighter than those in disparate clusters. This paper approaches community detection in graphs by constructing Markov random walks on the graphs. The mixing properties of the random walk are then used to identify communities. We use coupling from the past as an algorithmic primitive to translate the mixing properties of the walk into revealing the community structure of the graph. We analyze the performance of our algorithms on specific graph structures, including the stochastic block models (SBM) and LFR random graphs.

==> glodef.tex <==
% Theorem-like environments

\newtheorem{Theorem}{Theorem}
\newtheorem{Theorem*}{Theorem}

\newtheorem{Claim}{Claim}
\newtheorem{Claim*}{Claim}
\newtheorem{Corollary}[Theorem]{Corollary}
\newtheorem{CounterExample*}{$\overline{\hbox{\bf Example}}$}
\newtheorem{Definition}{Definition}
\newtheorem{Example}{Example}
\newtheorem{Example*}{Example}
\newtheorem{Exercise}{Exercise}
\newtheorem{Intuition*}{Intuition}
\newtheorem{Joke*}{Joke}
\newtheorem{Lemma}[Theorem]{Lemma}
\newtheorem{Lemma*}{Lemma}
\newtheorem{Observation}{Observation}
\newtheorem{Open problem}{Open problem}
\newtheorem{Proposition}{Proposition}
\newtheorem{Property}{Property}
\newtheorem{Question}{Question}
\newtheorem{Question*}{Question}
\newtheorem{Remark*}{Remark}
\newtheorem{Result}{Result}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
\def \bDefinition{\bthm{Definition}}
\def \eDefinition{\ethm{Definition}}
\def \eDefinitionp{\ethmp{Definition}}
\def \bExample   {\bthm{Example}}
\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bOpen      {\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \ePropertyp {\ethmp{Property}}
\def \bProposition  {\bthm{Proposition}}
\def \eProposition  {\ethm{Proposition}}
\def \ePropositionp {\ethmp{Proposition}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
\def \bRemark    {\bthm{Remark}}
\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}
\def \bObservation   {\bthm{Observation}}
\def \eObservation   {\ethm{Observation}}
\def \eObservationp   {\ethmp{Observation}}



\def \bSubexa    {\begin{subexa}}
\def \eSubexa    {\ethm{subexa}}
\def \eSubexap   {\ethmp{subexa}}

% Environments

\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{{}}

\newcommand{\problem}[1]{#1}
%\newcommand{\problem}[1]{}

%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
\newcommand{\solution}[1]{{\\ \bf Solution}\quad #1}
%\newcommand{\solution}[1]{#1}
%\newcommand{\solution}[1]{}

\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\modifiedfrom}[1]{(Modified from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}

\newcommand{\reportedby}[1]{Reported by #1.}
%\newcommand{\reportedby}[1]{}

\newcommand{\hint}[1]{Hint: #1}
%\newcommand{\hint}[1]{}
% Formating

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Equation formatting

\newcommand{\spreqn}[1]{{\qquad\text{#1}\qquad}}

% Handouts

\newcommand{\hohead}[3]{
\hfill\begin{minipage}{3.5cm}
\bf
#1\\ % class # (CSE20) (perhaps + term)
#2\\ % term (Fall 2K+1) or name (Alon Orlitsky)
%#3\\[2mm]
%Handout #3\\
\end{minipage}
}

\newcommand{\solhead}[3]{ % CSE20 -- Discrete Math; Fall 2K+1; 1
\begin{center}
  \Large #1\\[1ex]
  \normalsize #2\\[3ex]
  Solutions for Homework Assignment \##3\\
\end{center}
}

% Blackboard fonts

\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}} % \dN
%\newcommand{\QQ}{\mathbb{Q}} % \dQ
%\newcommand{\RR}{\mathbb{R}} % \dR
\newcommand{\ZZ}{\mathbb{Z}} % \dZ

% Numbers

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}
\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\RRp}{\realsp}
\newcommand{\integersp}{\ZZ^+}
\newcommand{\integerss}[1]{\ZZ_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cU     {{\cal U}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vec#1{{\overline{#1}}}

\def \veca  {{\vec a}}
\def \vecb  {{\vec b}}
\def \vecu  {{\vec u}}
\def \vecv  {{\vec v}}
\def \vecV  {{\vec V}}
\def \vecx  {{\vec x}}
\def \vecX  {{\vec X}}
\def \vecy  {{\vec y}}
\def \vecY  {{\vec Y}}
\def \vecz  {{\vec z}}

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctV  {{\vct V}}
\def \vctx  {{\vct x}}
\def \vctX  {{\vct X}}
\def \vcty  {{\vct y}}
\def \vctY  {{\vct Y}}
\def \vctz  {{\vct z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\bf #1}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish

% notes

%\definecolor{light}{gray}{.75}

\def \mynote#1{{}}

% marginal notes

\def \marcha{{\marginpar{CHNGD}}}
\def \marfix{{\#\marginpar{FIX \#}}}
\def \marnew{{\marginpar{NEW}}}
\def \marok{{\#\marginpar{\# OK?}}}

% qed's

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}
\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \set#1#2{{\{{#1}\upto{#2}\}}}

\def \setpmo   {\{\pm 1\}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations

\def \union  {\cup}
%\def \union  {\bigcup}
\def \unionl {\union\limits}
%\def \Union {\Bigcup} % want this
\def \Union  {\bigcup}
\def \Unionl {\Union\limits}

\def \inter  {\cap}
%\def \inter  {\bigcap}
\def \interl {\inter\limits}
\def \Inter {\Bigcap}
\def \Interl {\Inter\limits}

% Floors and Ceilings

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}


% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\mathrm{def}}{=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cas}{\stackrel{\mathrm{a.s.}}{\to}}

%\def \ed     {\,{\buildrel \rm def \over =}\,}
\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% notation

\def \pr     {{p}}
\def \Pr     {{\hbox{Pr}}}
\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}
\def \Sets#1{{\left\{#1\right\}}}

\def \inseg#1{{[#1]}} % use \intsgm instead
\providecommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations

\def \union  {\cup}
%\def \union  {\bigcup}
\def \unionl {\union\limits}
%\def \Union {\Bigcup} % want this
\def \Union  {\bigcup}
\def \Unionl {\Union\limits}

\def \inter  {\cap}
%\def \inter  {\bigcap}
\def \interl {\inter\limits}
\def \Inter {\Bigcap}
\def \Interl {\Inter\limits}

% Floors and Ceilings

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}

% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory


% equalities

%\def \ed     {\,{\buildrel \rm def \over =}\,}
\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }


%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% notation

\def \pr     {{p}}
\def \Pr     {{\hbox{Pr}}}
\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\def \contra {{\leftrightarrows}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces


% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

% operators

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}


% for old documents


% picture macros

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}

